SVI-DAG: A Structured Variational Inference Approach to Bayesian Causal Discovery

Bayesian causal discovery seeks to determine the posterior distribution of causal theories, which are interpreted as directed acyclic graphs (DAGs) that explain the observed data. The resulting posterior allows systematic reasoning regarding epistemic uncertainty within these theories. Nonetheless, finding such graphs is difficult due to identifiability problems and limited observational data. Furthermore, precisely approximating posterior over graphs is challenging given vast range of potential DAGs. Recent Bayesian approaches have addressed some of these challenges, yet they remain limited as they fail to encode dependencies between edges, and lack principled ways to incorporate domain knowledge as inductive biases during the search process. To overcome these limitations, we propose SVI-DAG, a structured variational inference approach to Bayesian causal discovery using observational data and prior beliefs that uses normalizing flows to model dependencies between edges, supporting expressive and multimodal posterior learning over DAGs. To mitigate mode seeking behaviour in evidence lower bound optimization and promote mode coverage, we use stein variational gradient descent to update the node potentials using a kernel in acyclicity space. We evaluate SVI-DAG against 5 state-of-the-art Bayesian DAG learning methods and demonstrate competitive performance in terms of both accuracy and uncertainty quantification.

==> figures/tikz_codes/figure3.tex <==
\begin{tikzpicture}[scale=1.2, >=stealth]

\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.18}   % add only if you don't already set a compat level
\definecolor{truedir}{RGB}{0,158,115}
\definecolor{revdir}{RGB}{213,94,0}
\definecolor{noedge}{RGB}{153,153,153}

\begin{groupplot}[
    group style={group size=2 by 1, horizontal sep=10mm, y descriptions at=edge left},
    xbar stacked,
    width=0.47\linewidth, height=3.4cm,
    xmin=0, xmax=100,
    xtick={0,25,50,75,100},
    xlabel={Posterior mass (\%)},
    symbolic y coords={Correct, Noninf., Incorrect},
    ytick=data,
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    title style={font=\footnotesize},
    bar width=9pt,
    enlarge y limits=0.4,
    every axis plot/.append style={draw=none},
]
\nextgroupplot[title={Linear (not identifiable)}]
\addplot[fill=truedir] coordinates {(0.0,Incorrect) (40.1,Noninf.) (83.2,Correct)};
\addplot[fill=revdir]  coordinates {(84.7,Incorrect) (42.5,Noninf.) (0.0,Correct)};
\addplot[fill=noedge]  coordinates {(15.3,Incorrect) (17.4,Noninf.) (16.8,Correct)};
\node[font=\tiny, text=white] at (axis cs:42.4,Incorrect) {84.7};
\node[font=\tiny]             at (axis cs:92.4,Incorrect) {15.3};
\node[font=\tiny, text=white] at (axis cs:20.1,Noninf.)   {40.1};
\node[font=\tiny, text=white] at (axis cs:61.4,Noninf.)   {42.5};
\node[font=\tiny]             at (axis cs:91.3,Noninf.)   {17.4};
\node[font=\tiny, text=white] at (axis cs:41.6,Correct)   {83.2};
\node[font=\tiny]             at (axis cs:91.6,Correct)   {16.8};
\nextgroupplot[title={Nonlinear (identifiable)},
    legend to name=priorlegend, legend columns=-1, area legend,
    legend style={font=\footnotesize,
      /tikz/every even column/.append style={column sep=8pt}}]
\addplot[fill=truedir] coordinates {(0.2,Incorrect) (80.3,Noninf.) (95.2,Correct)};
\addplot[fill=revdir]  coordinates {(13.3,Incorrect) (5.2,Noninf.) (2.1,Correct)};
\addplot[fill=noedge]  coordinates {(86.4,Incorrect) (14.5,Noninf.) (2.7,Correct)};
\legend{$X_1 \rightarrow X_2$ (true), $X_1 \leftarrow X_2$, $X_1 \independent X_2$}
\node[font=\tiny, text=white] at (axis cs:6.9,Incorrect)  {13.3};
\node[font=\tiny]             at (axis cs:56.7,Incorrect) {86.4};
\node[font=\tiny, text=white] at (axis cs:40.2,Noninf.)   {80.3};
\node[font=\tiny]             at (axis cs:92.8,Noninf.)   {14.5};
\node[font=\tiny, text=white] at (axis cs:47.6,Correct)   {95.2};
\end{groupplot}
\end{tikzpicture}

